Neural Network Quantization for Efficient Inference: A Survey

As neural networks have become more powerful, there has been a rising desire to deploy them in the real world; however, the power and accuracy of neural networks is largely due to their depth and complexity, making them difficult to deploy, especially in resource-constrained devices. Neural network quantization has recently arisen to meet this demand of reducing the size and complexity of neural networks by reducing the precision of a network. With smaller and simpler networks, it becomes possible to run neural networks within the constraints of their target hardware. This paper surveys the many neural network quantization techniques that have been developed in the last decade. Based on this survey and comparison of neural network quantization techniques, we propose future directions of research in the area.

==> schemes-table.tex <==
\begin{table*}[h]
    \caption{\label{tab:schemes} A qualitative comparison of binary, ternary, integer/fixed point, and mixed precision quantization schemes}
    \centering
    \begin{tabular}{p{3cm} p{3cm} p{4cm} p{4cm}}
        \hline
        \textbf{Quantization Scheme} & \textbf{Accuracy Loss} & \textbf{Advantages} & \textbf{Disadvantages} \\
        \hline
        Binary & High & \textbf{Low cost.} All arithmetic done via binary operations. $32 \times$ size compression rate. & \textbf{High accuracy loss.} Binary networks often incur around 10\% accuracy reductions.  \\
        \hline
        Ternary & Low - Moderate & \textbf{High compression rate.} Multiplications done via binary operations or capped at two multiplications per activation if using assymetric scaling factors. $16 \times$ compression rate. & \textbf{Floating point arithmetic}. For negligible accuracy loss, ternary networks use asymmetric floating point scaling factors, so they need to perform two floating point multiplications per activation. \\
        \hline
        Integer/Fixed Point & Low & \textbf{Integer arithmetic.} All arithmetic done via integer arithmetic, which is much cheaper than floating point arithmetic. & \textbf{Uniform precision.} For minimal accuracy loss, the networks are limited to the bitwidth of most sensitive layer, which is often 8 bits, so the compression rates are at most $4\times$. \\
        \hline
        Mixed Precision & Low & \textbf{Custom precision.} Quantization scheme for each layer or even row of weights is tailored to their precision sensitivity, reaping the benefits of binary, ternary, and integer quantization. & \textbf{Large search space.} The search space for which quantization scheme to use for each layer or weight row is exponential in the number of layers or weight rows, respectively. \\
        \hline
    \end{tabular}
\end{table*}
